A Holistic Approach to Interpretability in Financial Lending: Models, Visualizations, and Summary-Explanations

Lending decisions are usually made with proprietary models that provide minimally acceptable explanations to users. In a future world without such secrecy, what decision support tools would one want to use for justified lending decisions? This question is timely, since the economy has dramatically shifted due to a pandemic, and a massive number of new loans will be necessary in the short term. We propose a framework for such decisions, including a globally interpretable machine learning model, an interactive visualization of it, and several types of summaries and explanations for any given decision. The machine learning model is a two-layer additive risk model, which resembles a two-layer neural network, but is decomposable into subscales. In this model, each node in the first (hidden) layer represents a meaningful subscale model, and all of the nonlinearities are transparent. Our online visualization tool allows exploration of this model, showing precisely how it came to its conclusion. We provide three types of explanations that are simpler than, but consistent with, the global model: case-based reasoning explanations that use neighboring past cases, a set of features that were the most important for the model's prediction, and summary-explanations that provide a customized sparse explanation for any particular lending decision made by the model. Our framework earned the FICO recognition award for the Explainable Machine Learning Challenge, which was the first public challenge in the domain of explainable machine learning.

==> Old/main_old_please_update_Management-science_.tex <==
%\documentclass{article}


% if you need to pass options to natbib, use, e.g.:
% \PassOptionsToPackage{numbers, compress}{natbib}
% before loading nips_2018

% ready for submission
%\usepackage{nips_2018}

% to compile a preprint version, e.g., for submission to arXiv, add
% add the [preprint] option:
 %\usepackage[preprint]{nips_2018}

% to compile a camera-ready version, add the [final] option, e.g.:








% The \author macro works with any number of authors. There are two
% commands used to separate the names and addresses of multiple
% authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to
% break the lines. Using \AND forces a line break at that point. So,
% if LaTeX puts 3 of 4 authors names on the first line, and the last
% on the second line, try using \AND instead of \And before the third
% author name.



%\begin{document}
% \nipsfinalcopy is no longer used

%\maketitle



\section{Introduction}

%In 2018, the Fair Isaac Corporation (FICO) proposed a challenge to data science researchers: present an explainable model for predicting whether someone will default on a loan. FICO provided a dataset for the challenge and asked researchers to provide explanations for the global model, as well as local explanations (explanations for a given prediction). They also requested that the global model respect monotonicity constraints (increasing or decreasing) on several of the variables.

%\iffalse
%elaborate on the application; 

%- Predictive models for credit-risk evaluations 

%\fi

%In responding to this challenge, we considered the specific aspects of the dataset in our modeling approaches: 
%the FICO data are balanced between the two classes, most of the features are real-valued, and most importantly, each of the 23 features is itself interpretable. Because the features already come with good representation, the algorithm does not need to construct the representation. Generally, for data having this particular property,  perhaps with a small amount of feature engineering, most machine learning algorithms tend to have almost the same performance, including algorithms that produce globally interpretable models. Thus, we aimed to create a model that was fully and globally interpretable, %\citep{Ming},
%rather than to construct a black box.

%We call our globally interpretable model a \textit{two-layer additive risk model}. It was designed to resemble traditional subscale models, where the features are partitioned into meaningful subgroups, and the subgroup scores are later combined into a global model. Traditional subscale models are generally interpretable because they are decomposable into meaningful components, and because these models are usually linear with coefficients whose sign is positive for risk factors. Our model preserves these classical elements (decomposable, uses linear modeling, positive coefficients for risk factors), but inserts (interpretable) nonlinearities in several places to make the model more flexible and accurate. In particular, the algorithm transforms the original features into piecewise constant functions that monotonically increase (or decrease) if we constrain them to do so. Combinations of these piecewise constant functions form the subscales in the second layer of the model. The subscales are fed through a sigmoid nonlinearity, which has the effect of adding more perceptron-like flexibility to the model, but also makes the subscale scores more meaningful as their own ``mini-models;'' each subscale produces its own probability of defaulting on a loan. The subscales are combined linearly and sent through a sigmoid function to produce the final probability of defaulting on a loan.

%While working on this challenge, it is important to note that the guidelines asked for an explanation for each class of the global model, such as variable importance information. It did not necessarily ask for a model that is globally interpretable. Perhaps it could benefit FICO to have a global model that is \textit{not} interpretable (a ``secret sauce'')? It is not clear that even if there exists a globally interpretable model, such as the one we found, that it would be desirable for FICO to release it. Thus, we were not certain that we responded as much to FICO's needs as we did to its customers' needs when creating our competition entry. Thankfully, as it turned out, FICO actually did respond positively to the globally interpretable model.

%\textcolor{red}{In many real-life applications, we want to learn a predictive model that explains its decisions using predicates (i.e., decision factors). For example, when assessing the risk of cardiovascular diseases, we want a model that can explain why a particular patient is at high risk, using risk factors such as ``high blood pressure'' or ``high blood sugar.'' At the same time, we also want the model to respect our prior knowledge of how a particular feature should be related to an outcome: in cardiovascular risk assessment, we expect our model to assign higher risk to patients with higher blood pressure, because high blood pressure generally increases the risk of cardiovascular diseases'' \cite{kannel1996blood}.}

Lending decisions are important high-stakes decisions that can deeply affect people's lives. In accordance with both legal and ethical principles, financial firms are required to provide clear explanations for why a particular loan application was denied \cite{regulation2016general,???}. While many financial firms have developed machine learning models for assessing a client's credit risk, these models are often complicated black-box models, or they are proprietary (and are thus de facto black-box models for the loan applicants). Even when model explanations are provided, there can be a gap between the explanations for why a loan is denied and the actual computations of the model, because the explanations may be created \textit{posthoc}. 

New laws, such as the GDPR \cite{regulation2016general} are starting to protect the rights of individuals with respect to algorithmic decisions. While these laws develop and become more expansive, their impact could be heightened if decision support tools could be shown to be more effective, given the opportunity of transparency in the risk models. In order to determine the potential efficacy of such tools, we would first need to propose ways to build them. A new framework for transparent decision-making in lending decisions could potentially encourage the veil of secrecy to be lifted from these models, and provide an immediate alternative approach to current lending approaches once that veil is lifted.
%Perhaps our decision support tools become more useful if the models were public? 

In this paper, we ask the following question: if a lending model is not required to be proprietary, ideally what kind of decision-making tools would be useful for important loan decisions? We aim to answer this question by providing a holistic approach to fully transparent and interpretable lending decisions. In particular, our approach includes: (1) a globally transparent model for credit risk, (2) a ranking mechanism to find important factors, (3) globally-consistent ``summary explanations'' to show patterns in the model's predictions, (4) case-based explanations to show known similar cases that are predicted in the same way as the unknown test case, and (5) an online interactive visualization of the entire model. Let us describe these in more detail.

\textbf{The Global Model:} We call our globally interpretable model a \textit{two-layer additive risk model}. It was designed to explain its decisions using risk factors and to preserve the monotonic relationship between certain features and predicted risk. It resembles a traditional subscale model, where features are partitioned into meaningful subgroups, and the subgroup scores are later combined into a global model. Traditional subscale models are generally interpretable because they are decomposable into meaningful components, and because these models are usually linear with coefficients whose sign is positive for risk factors. Our model preserves these classical elements (decomposable, uses linear modeling, positive coefficients for risk factors), but inserts (interpretable) nonlinearities in several places to make the model more flexible and accurate. In particular, the algorithm transforms the original features into piecewise constant functions that monotonically increase (or decrease) if we constrain them to do so. Combinations of these piecewise constant functions form the subscales in the second layer of the model. The subscales are fed through a sigmoid nonlinearity, which has the effect of adding more perceptron-like flexibility to the model, but also makes the subscale scores more meaningful as their own ``mini-models;'' each subscale produces its own probability of risk. The subscales are combined linearly and sent through a sigmoid function to produce the final probability of risk.
Our two-layer additive risk model is a globally interpretable model. This means that
%the entire reasoning process of our model is accessible and can be easily explained to humans.
the entire reasoning process of our model is reflected in the full computation of the model, and can be easily explained to humans. 
%We applied our model to predicting credit risk. %In our credit risk application, we

\textbf{Important Factors:} Our global model also comes with a natural way to find important decision factors for why a loan is denied. \textcolor{red}{In particular, ???}

\textbf{Summary-Explanations:} Even though our global model is globally interpretable and thus can be explained on its own, we can also produce optional local \textit{summaries} of general trends in the global model. These are summaries rather than explanations (or \textit{summary-explanations}) in that they do not aim to reproduce the global model, only to show patterns in its predictions. The summary-explanation method we use (called \texttt{SetCoverExplanation}) is a model-agnostic explanation algorithm \cite{ShaposhnikRu18}. \texttt{SetCoverExplanation} solves a minimal set cover optimization problem \citep{feige1998threshold,feige1996threshold} to generate conjunctive rules that are consistent with all training cases. For instance, for a particular applicant's denied loan, a summary-explanation might say that ``all other 594 past applicants with average months in file below 48 were predicted to default on their loan.'' Summary-explanations can be constructed on a per-applicant basis.

\textbf{Case-based Explanations:} Given a previously unseen case, we can find known similar cases that are predicted in the same way as the previously unseen case by the global model.

\textbf{Interactive Visualization Tool:} Our interactive display shows the full computation of a two-layer additive risk model from beginning to end, without hiding any nonlinearities or computations from the user.\footnote{Anyone can interact with our tool at http://dukedatasciencefico.cs.duke.edu .} Risk factors are colored according to their contributions to the model. The form of our model lends itself naturally to explaining predictions using risk factors, and understanding monotonicity constraints, through the visualization.

To create an explanation of an individual prediction, our interactive display first highlights the factors that contribute most heavily to the final prediction of the global model. Second, it shows patterns produced by \texttt{SetCoverExplanation}.
Third, it provides case-based explanations. Our case-based reasoning method finds cases that are similar on important features to any current case that the user inputs.

Following related work in Section \ref{sec:related}, we provide the model in Section \ref{gen_inst}, \textcolor{red}{keep going}... . 
Ultimately the value of a decision support tool lies with the value it provides to its users. Our model was evaluated by domain experts at FICO, as part of the Explainable Machine Learning Challenge,\footnote{???} where it received the FICO recognition award. This recognition is an important indicator that our framework is on the path to what financial decision-makers would find useful and appealing.


\section{Related Work}\label{sec:related}

Many companies are now providing explainable AI technologies for lending. This includes Equifax's proprietary NeuroDecision Technology \cite{??}, and an approach published by Wells Fargo \cite{ https://arxiv.org/pdf/1806.01933.pdf}. Both Equifax's methodology and model is proprietary, and Wells-Fargo's model is also proprietary. Wells-Fargo's model cannot be used in practice as described because it does not seem to incorporate the monotonicity constraints that are required for lending (though it could be made to do so), along with other types of constraints one might require for practical decision-making. Monotonicity constraints are important, because as risk factors increase, the estimated risk should also increase. Traditionally, banks use a collection of subscale models that are each additive (linear in nonlinear transformations of the variables), because they are decomposable, interpretable, and obey monotonicity constraints \cite{??}. Our evidence suggests that additive subscale models may not lose accuracy over more complicated black box AI tools, which is a topic we explore later. 

There are a number of recent academic works in explainable credit risk modeling stemming from the 2018 Explainable Machine Learning Challenge
\textcolor{red}{The steffen link does not exist}
\cite{Sanjeeb2018, Rory2018, Steffen2018}.  \citet{Sanjeeb2018} used column generation to efficiently search over an exponential number of candidate conjunctive or disjunctive clauses without the need for heuristic rule mining. \citet{Rory2018} proposed positive counterfactuals \textcolor{red}{what's that?} and introduced several weighting strategies to generate more understandable counterfactuals. \citet{Steffen2018} created a multifaceted black-box model explanation to enhance the explainability of machine learning models and demonstrated their results with a beautiful visualization tool. However, none of these approaches produce globally interpretable models like ours, they all aim to explain a black box. We remark, however, that the instructions for the competition stated that one should create a black box and explain it, despite the fact that (as we found) it was not necessary to use a black box since the same performance level could be gained with an interpretable model.  

%Our approach contrasts with the common approach of explaining a ``black-box'' model.
%The issue raised above,
The distinction between explainability of a black box model, versus providing a globally interpretable model, is important, and there is a chasm between them in practice. Explanations can be problematic for several reasons \cite{Rudin19}. First, unless the global model is uniformly equal to the local model, the explanations will be sometimes incorrect, which makes it difficult to trust either the explanations or the global model itself. Second, posthoc explanations do not respect variable importance. Even if an explanation gives the same prediction as the global model, it could be inconsistent with the global model's actual calculations  \citep{guidotti2018survey}. Third, the explanation method might provide reasons that may be true for some cases but not others. For instance, a reason of ``too many accounts open'' may be used to deny someone a loan even if there is another person with the same number of open accounts who was offered a loan by the same global model. Analogously, explanations could be correct but misleading, offering reasons that are true but incomplete -- missing key information. Fourth, explanations may hide the processing of missing or incorrect data, which may influence the decision. All of these problems with explanations for black-box methods are reasons that consumers would benefit from globally interpretable models. 

As far as we know, all other entries in the 2018 Explainable Machine Learning Challenge provided a black box with posthoc explanations, as per the competition's directions. In the citation for the FICO Recognition Award received by the work described here, FICO acknowledged that the submission had gone above and beyond expectations with a fully transparent global model and a user-friendly dashboard to allow users to explore the global model and its explanations; in other words, it appears that the competition organizers (or other contestants) did not expect that the data could be explained by a globally interpretable model. The (false) belief that black box models must be more accurate than interpretable models can lead to serious problems for lending, given the stakes of the decisions being made about individuals.


%\footnote{Companies such as DivePlane are now grappling with this issue, where they do not, as of this writing, release code or demonstrations of their models, which are claimed not to be black boxes.}

With the new General Data Protection Regulation (GDPR) \citep{regulation2016general} in Europe, regulations such as ``right to an explanation,'' could still provide little incentive for companies to provide anything more than a modestly local explanation, even if a globally interpretable model existed. 



Monotonicity and other constraints are essential to both interpretability and legal requirements \cite{??} for lending models. However, typical machine learning methods cannot be easily adapted to handle 
\textcolor{red}{FIX ME Attempts to create globally interpretable models for financial, healthcare, or other high-stakes applications use mainly standard machine learning approaches (e.g., decision trees and support vector machines were used for bank direct marketing \cite{moro2011data, moro2014data}). Most of these standard methods cannot model 
the monotonic relationship between certain features and predicted risk. There are some works on decision tree learning methods that enforce (or improve) the monotonic relationship between features and outcome: these works either use pruning to remove subtrees that violate the monotonic relationship \cite{ben1989learning,ben1992automatic,feelders2003pruning}, or they include a regularization term that penalizes potential violation of the monotonic relationship in greedy splitting criteria \cite{ben-david1995monotonicity}. However, these methods either cannot optimize the accuracy while enforcing the monotonic relationship at the same time, or they cannot fully enforce the monotonic relationship. There are also works that find rule lists \cite{letham2015interpretable,wang2015falling,angelino2017learning,chen2018optimization}, but rules are not natural for datasets with many real-valued features. On the other hand, additive scoring models are natural for real-valued features and can easily preserve monotonicity between certain features and risk. In the past, such models were often created by domain experts. For example, the CHADS$_2$ score for predicting the atrial fibrillation stroke risk was created by a group of medical professionals \cite{gage2001validation}. There are recent works that used machine learning techniques to create medical scoring systems \cite{ustun2016supersparse, UstunRu2017KDD}. Our two-layer additive risk model differs from traditional scoring models in that it partitions features into meaningful subgroups (called \textit{subscales}) and includes a second layer that introduces more nonlinearities. The resulting model is a hybrid of additive scoring models and a small neural network, and is more expressive than traditional scoring models.}

%Attempts to create globally interpretable models for financial applications use mainly standard machine learning approaches (e.g., decision trees and support vector machines are used for bank direct marketing \citep{moro2011data, moro2014data}), which cannot accommodate FICO's monotonicity constraints. Some work finds optimal rules \citep{chen2018optimization}, but rules are not natural for datasets with many real-valued features, like FICO's data. Additive models are natural for real-valued features and can easily preserve monotonicity. %In contrast, our globally interpretable model adds some twist to standard machine learning models and allows for efficient gradient-based training.



%The interpretability of a machine learning model has often become a necessity instead of a luxury in many domains, especially with the recent movement of the GDPR that requires the ``right to explanation''. Domain experts in healthcare, judiciary systems, credit report systems, etc. need to understand a machine learning model in order to trust and use the predictions and get meaningful insights. 
%In this paper, we are interested in predicting credit risk performance. When a customer applies for a credit card, credit card companies would like to have some estimate of this person's risk of default, in order to decide whether to approve the application. Accurate predictions help credit card companies reduce the cost and obtain good customers. Meanwhile, domain experts would also like to understand the reasoning for a prediction instead of leaving all decisions to a black-box. Therefore, our goal in this paper is to design a system that makes accurate predictions and also enables users to understand the prediction. To do that, we first propose an interpretable predictive model and then design three explanation models of different forms.
%Various forms of interpretable models have been proposed in the literature, such as rule-based models \cite{}, scoring models \cite{} and etc. Rule-based models are designed to use a small subset of features to generate a prediction. Scoring models only allow linearity in the decision boundary. Here, we design an additive risk Model that provides more comprehensive insights from all features and allow non-linear interactions of the feature space. We design a fully interpretable model that combines the best of a traditional credit scoring system and a feed-forward neural network with one hidden layer. The features are partitioned into meaningful subgroups, each fed into a neuron to generate a risk score. The risk scores are then combined to produce the final output. This construction resembles a traditional additive credit scoring model; however, unlike traditional models, nonlinear transformations were used to generate subscale outputs.  


Why is it that for the FICO data, and for other datasets in finance and in many other domains, imposing constraints such as monotonicity, sparsity, or other forms of interpretability, do not necessarily hurt accuracy? This seems to depend on the representation of the data. For data that lie on manifolds in feature space (e.g., realistic images lie on a manifold in pixel space), neural networks seem to (currently) have an advantage over other techniques, but for most structured data with interpretable features (e.g., data from many criminal justice, healthcare, and finance applications), there seems to be no advantage from switching to neural networks. One modern theory, called the \textit{Rashomon set} theory, aims to explain why this is the case \cite{SemenovaRuPa19}. Specifically, it proposes that for these typical structured problems, a large set of approximately-equally-good models exist, and if this set is large enough, there should be models within that set that obey various constraints, such as interpretability, or monotonicity. If this theory is correct, it should not be surprising that we find interpretable models that are just as accurate as black box models, however, the existence of interpretable accurate models renders the black boxes (and the process of explaining them posthoc) unnecessary.


A possible objection to using transparent credit risk models is that an individual who is not credit-worthy may try to game the models to improve their credit score \citep[Goodhart's law][]{???}. However, the credit score should be aligned inversely with credit risk. Actions taken to increase credit score should actually lower credit risk; if this is not the case, the scoring system is not designed correctly. No one should be able to have bad credit and a good credit score simultaneously.


%We created an interactive display that shows the full computation of the model from beginning to end, without hiding any nonlinearities or computations from the user. Factors are colored according to their contribution to the global model. The form of our global model lends itself naturally to variable importance analysis, and understanding monotonicity constraints, through the visualization.

The novel elements of the work are (i) the form of the two-layer additive risk model, which lends naturally to sparsity, decomposability, visualization, case-based reasoning, feature importance, and monotonicity constraints, (ii) the interactive visualization tool for the model, (iii) the use of the \texttt{SetCoverExplanation} algorithm for high-support local conjunctive explanations, and (iv) the application to finance, indicating that black boxes may not be necessary in the case of credit-risk assessment.

A paper describing the competition entry appeared at the workshop associated with the competition \citep{ChenEtAlFICO2018}.

% Our vision for this competition entry was to create a fully interpretable global model that combines the best of a traditional credit scoring system and a feedforward neural network,
% %that is interpretable, like a traditional model that uses subscales, but is a fully optimized nonlinear machine learning model.
% without sacrificing any accuracy to gain interpretability (and indeed we did not\footnote{The accuracy achieved by our global model in a cross-validation test is 75\%, similar to other frequently used machine learning models.}). 
% To achieve this end, we created a model that is subdivided into 10 smaller interpretable isotonic regression models (subscales), that are combined at the end into a globally interpretable model.
% %have aggregated subsets of original input features into $10$ subscale scores, which are then nonlinearly transformed into $10$ estimates of default probability based on distinct customer information.
% %Each of the ten carefully selected subscales is meaningful on its own. In particular, each subscale estimates the probability of non-repayment based on distinct customer information.
% %The final prediction combines the subscale probabilities into an overall estimate. 

% %
%\textcolor{red}{maximum 8 content pages (including everything but reference; see previous email sent by Sijia)}

\section{Two-Layer Additive Risk Model and its Visualization}
\label{gen_inst}
We work with a dataset $\{(\mathbf{x}_i, y_i)\}_{i=1}^N$, where $\mathbf{x}_i \in \mathbbm{R}^P$ is a vector of features and the categorical features are binarized. The labels are indicators of defaulting on a loan: $y_i \in \{0,1\}$. Let $\mathcal{P}$ represent the set of features and $|\mathcal{P}| = P$.
We present the structure of our two-layer additive risk model (ARM).  %While in general, neural networks are hard to comprehend even with sparsity regularization applied, our model has carefully designed sparsity and monotonicity constraints that make the calculations easier to comprehend. 
Our additive model did not require quadratic terms, as \cite{Caruana13} did.

\subsection{Model Design}
The design of the model pursues interpretability by enforcing monotonicity constraint on features and meaningful grouping of features. Here we illustrate the two strategies.

First, to ensure monotonicity of the model with respect to any given features, we used step functions as our initial transformations of the features and constrained the coefficients of each feature's step functions to be non-negative. For instance, for a monotonically decreasing feature $x_{\cdot,p}$, the following features could be created: $b_{p,1}(x_{\cdot,p})=\mathbbm{1}[x_{\cdot,p} < 10]$, $b_{p,2}(x_{\cdot,p})=\mathbbm{1}[x_{\cdot,p} < 50]$, $b_{p,3}(x_{\cdot,p})=\mathbbm{1}[x_{\cdot,p} < 75]$, and $b_{p,0}(x_{\cdot,p})=\mathbbm{1}[x_{\cdot,p} \text{ is not missing}].$\footnote{We handle missing values also by creating binary indicator features for missingness.} To choose the proper thresholds for creating the binary features, we tried two different methods, both which use heuristic measures of ``purity'' of splitting the dataset by a specific candidate threshold and then choose a threshold yielding the ``purest'' group. One method uses information gain, which is a commonly used metric in classification algorithms such as decision trees, to measure how informative a feature is to predict a target variable. The other method directly uses predictive accuracy. In practice, we experimented with both approaches and then chose the one with the higher accuracy.
    %Note that all these non-missing binary features use one-sided intervals. %Details of how we convert the original features into the binary features are provided in Section~\ref{sec:training}.
    %The original $23$ continuous features were first encoded into binary features. If a feature $x_p$ is monotonically decreasing and has nonnegative support with missing values denoted by $-9$, $-8$, or $-7$, it could be encoded into the following binary features: $b_{p,1}=\mathbbm{1}[x_p=-9]$, $b_{p,2}=\mathbbm{1}[x_p=-8]$, $b_{p,3}=\mathbbm{1}[x_p=-7]$, and for non-missing values, $b_{p,4}=\mathbbm{1}[x_p < 10]$, $b_{p,5}=\mathbbm{1}[x_p < 50]$, $b_{p,6}=\mathbbm{1}[x_p < 75]$, $b_{p,7}=\mathbbm{1}[x_p < \infty]$. 
    
    Then the features are binary coded using selected thresholds. Note that all of these %non-missing binary 
    features use one-sided intervals. This choice was made because convex combinations of these step functions yield \textit{monotonic} piecewise constant functions. Specifically,
    %-- this is to ensure that when we fit a logistic regression model on the transformed binary dataset with risk performance labels (as we did when training the first layer subscale model), 
    by enforcing the constraints that the coefficients for $b_{p,1}$, $b_{p,2}$, and $b_{p,3}$ must be non-negative, we shall guarantee a monotonically decreasing relationship between the original continuous feature $x_{\cdot,p}$ and the subscale's predicted probability of default. Once the model is learned, the sum of the one-sided intervals becomes a piecewise constant function. For instance,
    \[
    f_p(x_{\cdot,p}) = \beta_{p,1} b_{p,1}(x_{\cdot,p}) + \beta_{p,2} b_{p,2}(x_{\cdot,p}) + \beta_{p,3} b_{p,3}(x_{\cdot,p}) + \beta_{p,0} b_{p,0}(x_{\cdot,p})
    \]
    can be equivalently written as
    \begin{eqnarray*}
    f_p(x_{\cdot,p}) &=& (\beta_{p,1}+\beta_{p,2}+\beta_{p,3}+\beta_{p,0})\mathbbm{1}[x_{\cdot,p}<10] \\ &&+ (\beta_{p,2}+\beta_{p,3}+\beta_{p,0})\mathbbm{1}[10 \leq x_{\cdot,p} < 50] \\
    &&+ (\beta_{p,3}+\beta_{p,0})\mathbbm{1}[50 \leq x_{\cdot,p} < 75] + \beta_{p,0}\mathbbm{1}[75 \leq x_{\cdot,p} ],
    \end{eqnarray*}
    which can be displayed as a traditional scoring system \citep{ustun2016supersparse,mdcalc}. We show a transformation like this in Figure~\ref{fig:ExternalRiskEstimate} for the ExternalRiskEstimate subscale. 
    %The transformation through the sigmoid is displayed for the user in a popup (middle). We also show a subscale that uses multiple features (right).
    \iffalse % previous
 \begin{figure}
        \centering
        \includegraphics[width=.25\linewidth]{ExternalRiskEstimate.png}\hspace*{5pt}
        \includegraphics[width=.22\linewidth]{FirstSubscale.png}\;\;
         \includegraphics[width=.45\linewidth]{SecondSubscale.png}
        \caption{The ``External Risk Estimate'' Subscale.  \textit{Left}: sum of thresholds, as a piecewise constant function, written as a scoring system. Because the value of the external risk estimate is less than 63, the person receives 1.799 points. \textit{Middle}: The transformation of points into a risk estimate, which is 81.9\% for this person. The risk estimate for the subscale is meaningful as its own ``mini-model'' of risk, based only on the EsternalRiskEstimate feature. \textit{Right}: A different subscale,  which uses multiple features. }
        \label{fig:ExternalRiskEstimate}
    \end{figure}
    \fi
    \begin{figure}
        \centering
        \includegraphics[width=.4\linewidth]{ExternalRiskEstimate.png}
        \caption{The ``External Risk Estimate" Subscale: sum of thresholds, as a piecewise constant function, written as a scoring system. Because the value of the external risk estimate is less than 63, the person receives 1.799 points.}
        \label{fig:ExternalRiskEstimate}
    \end{figure}    

    
    If coefficients $\beta_{p,1}$, $\beta_{p,2}$, and $\beta_{p,3}$, are nonnegative, the function $f_p$ is nonincreasing. 
    If instead, we would like to constrain $f_p$ to be monotonically increasing, we reverse the above one-sided inequalities ``$<$" into ``$>$". Of course, if a feature $x_p$ has no desired monotonicity, we drop non-negativity constraints from the optimization problem defined by the learning algorithm (to be discussed momentarily).
    


Using domain knowledge obtained from the data description, we partitioned the features $\mathcal{P}$ into different sets for the subscales, inducing sparsity in the first layer of the model and its connectivity to the input layer. Each subset of features is sent to one node which computes a subscale. Denote the feature subsets as:
\begin{equation*}
    \mathcal{P} = \cup_{k=1}^K\mathcal{P}^{[k]},
\end{equation*}
where a subset of features $\mathcal{P}^{[k]}$ is sent to a subscale. There are between 1 and 4 of the original features combined per subscale, yielding a total of 10 subscales to represent the original 23 features.
Each subscale can be interpreted as a miniature model %($L^2$-regularized logistic regression model) 
    for predicting the probability of failure to repay a loan, using only the features designated for the subscale. %In Figure~\ref{fig:SecondSubscale}, we see the four original features that constitute the ``Delinquency'' subscale. 
    The output of the subscale is a probability, denoted by $r^{[k]}$ for subscale $k$, which is simply a sigmoid transformation of the score, 
    \begin{equation*}
        %r^{[k]}(\mathbf{x}) = \sigma\left(\beta_0^{[k]} + \sum_{p\in \mathcal{P}^{[k]}}\beta_p^{[k]} {x}_{i,p}\right),
        r^{[k]}(\mathbf{x}) = \sigma\left(\sum_{p\in \mathcal{P}^{[k]}} f_p(x_{\cdot,p})\right) = \sigma\left(\sum_{p\in \mathcal{P}^{[k]}} \sum_{l=0}^{L_p} \beta_{p,l} b_{p,l}(x_{\cdot,p})\right),
    \end{equation*}
where $\sigma(\cdot)$ represents a sigmoid function and $L_p$ is the number of binary features created for feature $p$ (not counting the special indicator for non-missing values).

Finally, the subscale results are linearly combined and again nonlinearly transformed into a final probability of failure to repay a loan. The contribution of each subscale to the final prediction can be easily observed by its weighted output.


\subsection{Training the Model}
The simplest way to train coefficients %$\boldsymbol{\beta}^{[k]} = \{\beta_0^{[k]}, \beta^{[k]}_p\text{ for } p \in \mathcal{P}^{[k]}\}$
$\boldsymbol{\beta}^{[k]} = \{\beta_{p,l}\text{ for } p \in \mathcal{P}^{[k]}, l \in [0, L_p] \}$
is to treat each $r^{[k]}$ as an independent classification model with the $\{y_i\}_{i=1}^N$ being the target variables, using regularization (e.g., $\ell_2$) to prevent overfitting, and positivity constraints on the thresholds to enforce monotonicity. A slightly more complicated way to train is to optimize for a combination of accuracy for the subscales and accuracy for the global model. On our data, these two methods tended to produce almost identical results. An image of the full model is shown in Figure~\ref{fig:FullModel}, where the colors indicate the final contribution to the combined score. Red indicates more likely to default on the loan. The 23 feature values can be entered on the left, and clicking on any of the ten subscales (in the second colored layer) reveals a pop-up window with the calculation, as shown in Figure~\ref{fig:subscales} for two subscales. The final combination of features is shown in Figure~\ref{fig:FullModel} (right panel). Figure~\ref{fig:AccuracyPlot} shows that our global model does not lose accuracy over other machine learning techniques, despite being constrained to be interpretable. The accuracy results were obtained by averaging test accuracy figures of five random $80\%:20\%$ training-test splits. Our final model was trained on the entire dataset.
    \begin{figure*}[t]
    \centering
    \includegraphics[width=.65\linewidth]{GlobalModel.jpg}
    \includegraphics[width=.34\linewidth]{CombinedModel.png}
    \caption{\textit{Left}: Snapshot of visualization tool showing the global model. Colors indicate contribution to the final score. The 23 feature values are entered on the left. \textit{Right}: Final combined score pop-up.}
    \label{fig:FullModel}
\end{figure*}
%
    \begin{figure*}
        \centering
        \includegraphics[width=.3\linewidth]{FirstSubscale.png}\;\;
         \includegraphics[width=.61\linewidth]{SecondSubscale.png}
        \caption{The ``External Risk Estimate'' and ``Delinquency'' Subscales.  \textit{Left}: The transformation of points into a risk estimate, which is 81.9\% for this person. The risk estimate for the subscale is meaningful as its own ``mini-model'' of risk, based only on the ExternalRiskEstimate feature. \textit{Right}: A different subscale,  which uses multiple features. }
        \label{fig:subscales}
    \end{figure*}
    %
\begin{figure}[t]
\centering
%\fbox{
\includegraphics[width=\linewidth]{table_sorted3.jpg}
%\includegraphics[width=0.547\linewidth]{table_sorted3.jpg}
%}
%\fbox{
%\includegraphics[width=0.45\linewidth]{table_legend.jpg}
%}
\caption{The accuracy of our model compared to other common machine learning models.}
\label{fig:AccuracyPlot}
\end{figure}

\iffalse
\begin{figure}
\centering
\fbox{\includegraphics[width=0.45\linewidth]{table_legend.jpg}}
\caption{The accuracy of our model compared to other common machine learning models.}
\label{fig:AccuracyPlot2}
\end{figure}
\fi


\subsection{Variable Importance}
Our two-layer additive risk model comes naturally with a way to identify a list of factors that contribute most heavily to the final prediction.
Table~\ref{tab:ImportantFeatures} shows a list of four factors that are important for predicting observation ``Demo 1''  to have $95.2\%$ risk of default (i.e., bad risk performance). 

\begin{table*}[]
    \centering
    \caption{An example of the most important contributing factors learned for observation ``Demo 1'' }
    \begin{tabular}{c|l}
\toprule
         & \multicolumn{1}{c}{\textbf{Most important contributing factors}} \\ \hline 
      1   & MaxDelq2PublicRecLast12M is 6 or less (from the most important subscale, Delinquency)\\ 
      2 & PercentTradesNeverDelq is 95 or less (from the most important subscale, Delinquency)\\ 
      3 & AverageMInFile is 48 or less (from the second most important subscale, TradeOpenTime) \\ 
      4 & AverageMInFile is 69 or less (from the second most important subscale, TradeOpenTime) \\
         \bottomrule
    \end{tabular}
    
    \label{tab:ImportantFeatures}
\end{table*}% The most important contributing factors to predicting bad risk performance are listed in figure. 
%\begin{figure}
% \centering
%  \fbox{\includegraphics[width=0.95\linewidth]{ImportantFeatures.png}}
%  \caption{Most important contributing factors.}
%  \label{fig:ImportantFeatures}
%\end{figure}
%\iffalse
%\begin{tcolorbox}
%\begin{enumerate}
%    \item $MaxDelq2PublicRecLast12M$ is $6$ or less (from the most important subscale, Delinquency)
%    \item $PercentTradesNeverDelq$ is $95$ or less (from the most important subscale, Delinquency)
%    \item $AverageMInFile$ is $48$ or less (from the second most important subscale, TradeOpenTime), and
%    \item $AverageMInFile$ is $69$ or less (from the second most important subscale, TradeOpenTime). 
%\end{enumerate}
%\end{tcolorbox}
%\fi
To identify the factors, we first identify the most important two subscales and then the most important factors within each subscale.
The importance of each subscale in the final model is determined by its weighted score, which is the product of the subscale's output and its coefficient -- the larger the product, the larger the contribution of the term in the final risk. %For a test case that predicts bad risk performance, the top two subscales are the ones with the largest products. For a test case that predicts good risk performance, the top two subscales are the ones with the smallest products. 
%\textcolor{red}{This is Tong: Consider using Table 1 instead of Figure 3? too many figures already}

For example, for ``Demo 1'', the two most important subscales are Delinquency (with points of 1.973) and TradeOpenTime (with points of 1.947). Then, within each of the two subscales, we find two factors that contribute the most to that particular subscale's risk score. 
%Similar to identifying important subscales, 
The two most important factors for each subscale are determined likewise by the product of the coefficient of each binary feature and the value of the binary feature itself. %For a test case that predicts bad risk performance, the top two factors within an important subscale are given by the binary features with the largest products. For a test case that predicts good risk performance, the top two factors within an important subscale are given by the binary features with the smallest products. 
We finally output those binary features and their corresponding values as the most important contributing factors to the prediction made by our model.

The factors are grouped by subscales and are displayed in decreasing order of importance (within each important subscale) to the global model's predictions.

%and can be used to highlight aspects of the application that entails risk of defaulting. Note that other factors may still impact the prediction made by the model.

% The factors are displayed in decreasing order of importance to the global model's predictions. 
% We applied a customized training procedure to provide interpretability through {sparsity} and {monotonicity}:
% \begin{itemize}
%     \item Sparsity -- The resulting network is very sparse, with each node in the input layer feeding into a single node in the first layer. This structure aggregates the original $23$ features into $10$ subscales that capture distinct aspects of a customer's behavior. There are only a small number of discretization levels associated with each feature. The contribution of each subscale to the final prediction can be easily observed by its weighted output (which is colored red to green in the visualization).  

   % \item Monotonicity -- %We implemented a constrained training procedure that preserves the monotonicity of risk prediction with respect to changes in various features. 
    %such as  $b_{j,4}=\mathbbm{1}[x_j < 10]$.  <-- I suspect  it's a typo


% \end{itemize}


%Monotonicity constraints are enforced during learning; we discuss the formulation that enabled monotonicity with respect to these step functions shortly.  
%There are two important sources of nonlinearity: the initial transformation of features into step functions, and the sigmoid transformation of the linear combination of features. 
     
%, users can click on the subscales to view the calculation. None of the calculations are hidden to the user -- all nonlinearities are displayed. Figure~\ref{fig:subscales} shows examples of the subscales calculated for ???

% \begin{figure}[h]
% \begin{center}
% \includegraphics[scale=.75]{GlobalModel.jpg}
% \end{center}
% \caption{The global model. \label{fig:global}}
% \end{figure}


% \begin{itemize}
% \begin{figure}[h]
%   \fbox{\includegraphics[width=.7\linewidth]{FirstSubscale.png}}
%   \caption{The subscale ``ExternalRiskEstimate.''}
%   \label{fig:FirstSubscale}
% \end{figure}

%     \item \textbf{Initial transformation}: The $23$ original features are transformed into $182$ piecewise constant features, where missing values were converted to binary features. Each original feature contributes to one of the 10 subscales.
    
%     Figure~\ref{fig:FirstSubscale} shows how the (original) feature ``ExternalRiskEstimate'' is transformed into 8 binary features (e.g., one of the binary variables is an indicator specifying whether $0 \leq ExternalRiskEstimate\leq 63$). The individual whose score is being displayed in the figure has ExternalRiskEstimate between 0 and 63, and thus received 1.799 points for this feature.

% \begin{figure}[h]
%   \fbox{\includegraphics[width=.7\linewidth]{SecondSubscale.png}}
%   \caption{The subscale ``Delinquency''.}
%   \label{fig:SecondSubscale}
% \end{figure}


%     \item \textbf{First layer (subscale creation)}: 


% \begin{figure}
%   \fbox{\includegraphics[width=\linewidth]{CombinedModel.png}}
%   \caption{Output of global model.}
%   \label{fig:CombinedModel}
% \end{figure}


%     \item \textbf{Second layer (final risk estimation)}:

% \end{itemize}




% SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection*{Design principles}
% Our model is a feedforward neural network (NN). While in general, fully connected NNs are hard to comprehend even when sparsity regularization is applied, our model is a two-layer additive model with carefully designed sparsity and monotonicity constraints, which makes the calculations easier to comprehend. 
%\subsection{How we trained the model}\label{sec:training}

%The model was trained as follows.
%\begin{itemize}
%\item \textbf{Input transformation}: 

%The coefficients of the first layer were estimated using non-negativity (or non-positivity) constraints to ensure monotonicity. To capture non-linear dependencies, the original continuous features were encoded using binary features. For example, for a feature $x_i$ whose support is $[0,100]$ with missing values denoted by -9, the following 4 binary features could have been constructed: $b_1=\mathbbm{1}[x_i=-9]$, and for non-missing values, $b_2=\mathbbm{1}[x_i\leq 10],b_3=\mathbbm{1}[x_i\leq 50]$, and  $b_4=\mathbbm{1}[x_i\leq 75]$. Enforcing the coefficients $b_2$,  $b_3$, and $b_4$ to be non-negative guaranteed a monotonic relation between the original continuous feature value and the respective subscale.

%\item \textbf{First layer (subscale creation)}: Since each subscale model is an $L^2$-regularized logistic regression model whose input is a subset of binary features and whose output is a predicted probability of default based on this subset of binary features, we train each subscale model using a convex solver that minimizes the $L^2$-regularized logistic loss, subject to the appropriate non-negativity constraints for non-missing binary features whose original features have desired monotonicity property (explained above). 

%\item \textbf{Second layer (final risk estimation)}: Another $L^2$-regularized logistic regression model with non-negativity constraints was trained on the subscale probabilities to predict the final risk. Note that there is a monotonically increasing relationship between each subscale probability and the final predicted probability of default, so the non-negativity constraints should be enforced for every coefficient of the model (but not the bias).

%This preserved the monotonicity of the risk estimation with respect to the original features.
%\end{itemize}





%and can be used to highlight aspects of the application that entails risk of defaulting. Note that other factors may still impact the prediction made by the model. 
% \subsection{Case-based explanations:} The visualization contains a table showing the current case (top row) and previous cases that are most closely related to the current case (all other rows). All of the presented cases satisfy the rule-based explanations from \texttt{SetCoverExplanation}. Cases are sorted according to a distance metric that counts the number of identical features in the binary representation. See Figure~\ref{fig:CaseBased} for example case-based explanations. 


% These rules are generated by solving a Mixed Integer Program (MIP) using $\text{Gurobi}^{\text{(c)}}$. 
% The MIP formulation relies on key observations about binary feature spaces: 
% \begin{enumerate}
%     \item A subset of features and respective binary values forms a conjunctive rule.
%     \item The conjunctive rule must agree with the examined case.
%     \item All past cases with opposite predictions by the model must not satisfy the rule so that the explanation would remain globally consistent.  
% \end{enumerate}
% These properties imply that finding the minimal set of rules is in fact a \href{https://en.wikipedia.org/wiki/Set_cover_problem}{\textit{minimal set cover problem}}:
% \begin{enumerate}
%     \item Nodes correspond to cases.
%     \item Sets are a collection of cases that do not satisfy the rule. Each set is defined using a binary feature and its respective value.
    
%     %where sets are bijectively determined by features and their respective binary values (there is a 1-1 correspondence between sets and their features and their values), and
%     \item The objective is to minimize the number of features that comprise the rules. 
% \end{enumerate}
% After solving an initial minimal set cover problem, \texttt{SetCoverExplanation} seeks additional solutions that improve \textit{support} (that is, the number of previous cases that satisfy these rules) subject to constraints on the sparsity of the explanation. This is accomplished using a modification of the minimal set cover formulation. Maximizing support while constraining sparsity improves coverage and reliability of the explanation while maintaining interpretability. 

% Computing consistent explanations require solving a MIP which could lead to running-times of up to a minute (this could be tuned to improve running time or quality of the resulting solution). Nevertheless, computing explanations instantly are only required for testing purposes, and we expect that in an actual deployed system, explanations for most cases one would encounter online could be pre-computed offline, stored, and retrieved (memorized).

% %\item \textbf{Case-based explanations:} The visualization contains a table showing the current case (top row) and previous cases that are most closely related to the current case (all other rows). The distance metric used for identifying closely related cases is determined by the global model; features that are more important for the global model are weighted more highly in the distance metric. 
% %The cases are ordered according to decreasing order of similarity. Similarity is measured using the Values that are similar to the examined case are highlighted; these are values that contribute the same amount to the global model as the present examined case. All of the presented cases satisfy the rule-based explanations from \texttt{SetCoverExplanation}. See Figure~\ref{fig:CaseBased} for example case-based explanations. 




% \begin{figure}
%   \fbox{\includegraphics[width=\linewidth]{CaseBased.png}}
%   \caption{Case-based explanations.}
%   \label{fig:CaseBased}
% \end{figure}



% \subsection{Consistent rule-based explanations}




\section{Consistent rule-based explanations with \texttt{SetCoverExplanation}}

As noted earlier, in addition to predicting risk using a globally interpretable model, we generate consistent rules that summarize broad patterns of the classifier with respect to the data. They do not explain the global model's computations; instead, they provide useful patterns, which has been a popular form of explanation in the state-of-the-art literature on model explanations \citep{lakkaraju2017interpretable,guidotti2018local,ribeiro2018anchors}. As an example, consider Observation 6 in the FICO dataset, for which the global model predicts a high risk of default. \texttt{SetCoverExplanation}  returns the following rule-based summary-explanation that includes Observation 6:\vspace*{5pt}


\noindent\fbox{%
    \parbox{0.45\textwidth}{%
        For \textit{all} 700 people where: 
        \begin{itemize}
            \item ExternalRiskEstimate$\leq 63$ , and
            \item  NetFractionRevolvingBurden$\geq 73$, 
        \end{itemize}
         the global model predicts a high risk of default.
    }%
}


\texttt{SetCoverExplanation} asserts that our global model predicts high-risk for \textit{all} of the 700 previous cases that satisfy these rules. Therefore these rules are \textit{globally consistent}. In contrast, explanations (from other methods) that are not consistent may hold for one customer but not for another, which could eventually jeopardize trust.  

\iffalse
\textcolor{red}{fix me}
Suppose that for a given observation our global model predicts high-risk of default, and that the following rules are found:
% \iffalse
 %\begin{tcolorbox}

 For \textit{all} 700 people where: 
 \begin{itemize}
     \item $ExternalRiskEstimate\leq 63$ , and
     \item  $NetFractionRevolvingBurden\leq 73$, 
 \end{itemize}
 the global model predicts high-risk of default.
 %\end{tcolorbox}
% \fi
% \begin{figure}
% \centering
%   \fbox{\includegraphics[width=0.95\linewidth]{RuleBased_NoSupport.png}}
%   \caption{Rule-based explanations.}
%   \label{fig:RuleBased}
% \end{figure}
 \texttt{SetCoverExplanation} asserts that our global model predicts high-risk for \textit{all} of the 594 previous cases that satisfy these rules (including the examined case). Therefore these rules are \textit{globally consistent}. In contrast, explanations (from other methods) that are not consistent may hold for one customer but not for another, which could eventually jeopardize trust. 
\fi


%\textcolor{red}{Yaron: should we drop the paragraph below to save space?}\\

In what follows, we formalize the discussion on consistent rules and put it into concrete mathematical terms. 
After defining rules in Section~\ref{sub:rules_notation}, we address aspects of optimization in Section~\ref{sub:rules_optimization}. In Section~\ref{sub:consistent-cases} we describe how to use consistent rules to identify similar cases for case-based explanations.




\label{headings}
\subsection{Notation and definitions}\label{sub:rules_notation}

Consider a $P$-dimensional binary data set $\{(\mathbf{x}_i, y_i)\}_{i=1}^N$, that is, $x_{i,p}\in\{0,1\}$ for every $i$ and $p$. Let $h^M:\{0,1\}^P\rightarrow \{0,1\}$ denote a classifier that was trained using the dataset, and let $\textbf{y}^M$ denote the vector of labels generated by the model $h^M$ (the super-script $M$ stands for {model}). 

Assume $\mathcal{P}'\subseteq \mathcal{P}$ is a subset of features and ${y}\in\{0,1\}$ is a label. The \textit{rule} $\mathcal{P}'\Rightarrow {y}$ describes the following binary function/classifier:
\[ h^{\mathcal{P}'\Rightarrow {y}}\left(\textbf{x}\right) =
  \begin{cases}
    {y}       & \quad \text{if } \left(\prod_{p\in \mathcal{P}'} x_{\cdot,p}\right)=1 \\
    1-{y}     & \quad \text{otherwise.}
  \end{cases}
\]
That is, for a given observation $\textbf{x}$, the rule $\mathcal{P}'\rightarrow {y}$ predicts ${y}$ based on the projection of the observation onto the subspace of features $\mathcal{P}'$; specifically, by applying a logical AND operator on the subset of features in $\mathcal{P}'$. 

Let $\textbf{x}_e, y_e$ denote an observation and the respective model prediction that we wish to create a rule for. We say that the rule $\mathcal{P}'\Rightarrow y_e$ provides a \textit{consistent summary-explanation} for $\textbf{x}_e, y_e$ if the following conditions are met: 
\begin{enumerate}
\item (Relevance) $x_{e,p}=1$ for every $p\in \mathcal{P}'$.
\item (Consistency) For every observation $\textbf{x}_i$ for which $x_{i,p}=1$ for all $p\in \mathcal{P}'$, it must also hold that $y^M_i=y_e$.
%\item \textcolor{red}{(Consistency) When $x_{e,p}=1$ for every $p\in \mathcal{P}'$, it must also hold that $y^M_i=y_e$ for every observation $\textbf{x}_i\in\textbf{X}$ where  $x_{i,p}=1$ for every $p\in \mathcal{P}'$.} 
\end{enumerate}
The second condition establishes consistency by enforcing all observations in the dataset to agree with the rule, in the sense that all observations $i$ for which the binary variables in $\mathcal{P}'$ are true are similarly labeled by the global model $M$ as $y_i^M=y_e$. 

We measure the quality of a rule $\mathcal{P}'\rightarrow {y}$ using two criteria:
\begin{itemize}
\item \textit{Sparsity} -- the cardinally of $\mathcal{P}'$, that is, $|\mathcal{P}'|$. This captures to a certain degree the level of interpretability of the rule. 
\item \textit{Support} -- the number of observations in the dataset that satisfy the rule, namely $|\{\textbf{x}_i:\left(\prod_{p\in \mathcal{P}'} x_{i,p}\right)=1\}|$. This serves as a measure of coverage for the applicability of the rule. 
\end{itemize}

\iffalse
Ideal rules are sparse and have large support. However, the dataset may not be homogeneous and some observations may be more difficult to interpret than others. In this case, if only rules with low sparsity and support can be extracted, in which case human intervention may be needed.  
\fi

Note that the fact that the above definitions apply only to rules where features are equal to 1 (and not 0) may seem to be a limitation. However, one can easily extend the feature space by adding binary features that are equal to the complements of the original features, that is, by adding $\textbf{X}^c=1-\textbf{X}$. In this case, rules that contain complement features can be interpreted as rules where an original feature is equal to 0. 
In what follows, we assume that the design matrix $\textbf{X}$ is of dimensions $N\times 2P$ and includes both the original and complement matrices: $[\textbf{X},\textbf{X}^c]$. 
%However, for ease of presentation in what follows we only discuss rules where features are equal to 1. 


\subsection{Optimization}\label{sub:rules_optimization}

We now describe the formulation of multiple algorithms to generate rules that achieve the objectives of high sparsity and support. %These formulation draw on ideas for the minimal set cover problem.

\iffalse
\paragraph{Existence and necessary condition.}
According to the first condition of consistent rules, $x_{e,p}=1$ for each feature $p\in \mathcal{P}'$. Therefore the rule $\mathcal{P}_e\Rightarrow y_e$, where $\mathcal{P}_e = \{p:x_{e,p}=1\}$,  satisfies condition 1. Note that if there exists an observation $i$ for which $\textbf{x}_i=\textbf{x}_e$ and $y_i\neq y_e$, then there are no consistent rules as condition 2 is violated. Otherwise, the rule $\mathcal{P}_e\Rightarrow y_e$ is consistent. 
However, the sparsity of this rule is the worst possible, and its support is very likely to be 0. Nevertheless, existence can be easily verified. 
\fi

\paragraph{Optimizing sparsity.}
Let $b_p$ denote a binary decision variable that indicates whether $p\in \mathcal{P}'$.
Denoting $\mathcal{P}_e\overset{\Delta}{=}\{p:x_{e,p}=1\}$ as the largest set of features that ``agree'' with observation $\textbf{x}_e$ allows us to write Condition 1 as $\mathcal{P}'\subseteq \mathcal{P}_e$. Therefore, we need only consider variables $p$ for which $p\in \mathcal{P}_e$. In order for Condition 2 to hold, observations with labels different from $y_e$ must not satisfy the rule $\mathcal{P}'\Rightarrow y_e$. That is, for each such observation $i$, a feature $p\in \mathcal{P}_e$ must be selected for which $x_{i,p}=0$. Each feature $p$ therefore covers a set of observations with opposite labels, and a feasible solution must cover all observations whose labels are different from $y_e$. This is an instance of the \textit{Minimal Set Cover Problem} \citep{feige1998threshold,feige1996threshold}.

More formally, let $A_p\subseteq\{1,\ldots,N\}$ denote the (constant) set of observations $i$ that satisfy $x_{i,p}=0$. Finding a rule with optimal sparsity is the solution to the following optimization problem: 
\begin{equation}\label{eq:MaxSparsity}
\begin{array}{ll@{}ll}
\text{minimize}  & \displaystyle\sum\limits_{p\in \mathcal{P}_e} b_{p}      &\\
\text{subject to}& \displaystyle\sum\limits_{p\in \mathcal{P}_e} b_{p} \cdot \mathbbm{1}[\textbf{x}_i\in A_p]   & \geq 1,      &i\in\{i: y^{M}_i\neq y_e\}\\
&b_p \in\{0,1\} & & p\in \mathcal{P}_e.
\end{array}
\end{equation}

We briefly note that we conducted a computational study on the FICO dataset where sparse explanations were generated for each of the 10K observations, based on all other observations. The running time consistently took less than 7 seconds, and the average sparsity was under three features. 
\iffalse
Figure~\ref{fig:FrequencyvsSparsity} contains a histogram of the optimal sparsity per explanation in our global model. 


\begin{figure}
\centering
  \fbox{\includegraphics[width=.3\linewidth]{FrequencyvsSparsity.png}}
  \caption{The number of features per rule-based explanation in the FICO dataset.}
  \label{fig:FrequencyvsSparsity}
\end{figure}
\fi


\paragraph{Optimizing support.}
Formulation~(\ref{eq:MaxSparsity}) can be extended to incorporate support by adding a binary decision variable $r_i$ (and an appropriate linear constraint) for each observation that indicates that the rule applies to the respective observation. 
%Using these variables, the objective can be set to maximize their summation. To ensure correctness, additional constraints must be added to ensure that \textcolor{red}{HUH??? these observations are not covered by any of the features (and therefore the rule applies to them).} %Such constraints were implemented using the ``Big M method.'' 
An additional constraint was added to limit the number of features to a predefined constant MAX\_SPARSITY in the resulting rule. 

\iffalse
\textcolor{red}{as given by the following formulation:
\begin{equation}\label{eq:MaxSupport}
\begin{array}{ll@{}ll}
\text{maximize}  & \displaystyle\sum\limits_{i\in 1,\ldots,N} r_i      &\\
\text{subject to}& \displaystyle\sum\limits_{p\in \mathcal{P}_e} b_{p} \cdot \mathbbm{1}[\textbf{x}_i\in A_p]   & \geq 1,      &i\in\{i: y^M_i\neq y_e\}\\
&b_p \in\{0,1\}, & & p\in \mathcal{P}_e\\
& \displaystyle\sum\limits_{p\in \mathcal{P}_e} b_{p} \cdot \mathbbm{1}[\textbf{x}_i\in A_p]   & \leq |\mathcal{P}_e|\cdot (1-r_i),      & i\in 1,\ldots,N\\
&r_i \in\{0,1\}, & & i\in 1,\ldots,N\\
& \displaystyle\sum\limits_{p\in \mathcal{P}_e} b_{p} \leq \text{MAX\_SPARSITY}
\end{array}
\end{equation}
}
\fi 

%Note that the addition of $\mathcal{O}(N)$ variables and constraints increases the running time and therefore a timeout is set to ensure quick running time. 
We experimented with our formulations by generating summary-explanations on the FICO dataset. We first solved Formulation~\ref{eq:MaxSparsity}, and set its solution as the value of MAX\_SPARSITY in the modified formulation that optimizes support. We then increased the value of MAX\_SPARSITY by 1 and 2 to relax the respective constraint, in order to improve the support size (at the cost of worse sparsity).

We generated summary-explanations (where we maximized support) for all observations in the FICO dataset. The average number of features in each explanation did not change (comparing with the optimal sparsity) and was equal to 2.9 when MAX\_SPARSITY was set to the solution of Formulation~\ref{eq:MaxSparsity}; sparsity slightly worsened to 3.6 and 4.4 when MAX\_SPARSITY was increased by 1 and 2, respectively. We also found that the number of summary-explanations for which the support is less than 10 was 9.7\% of all observations for the solution given by Formulation~\ref{eq:MaxSparsity}, and was equal to 4.7\%, 1.2\%, and 0.2\% of all observations for the maximal support solution when  MAX\_SPARSITY was increased by 0, 1, and 2, respectively. Clearly, this indicates a trade-off between support and sparsity; when the constraint on MAX\_SPARSITY is relaxed, the cardinality of the rule increases and the rule becomes less interpretable, however, at the same time support increases which improves the confidence in the resulting rule. Overall, the average cardinality is nicely low, and the support is reasonably high.

\iffalse
The results are summarized in Table~\ref{tab:comparison_rules}. The table displays the average cardinality and support for each optimization problem. It also shows the number of observations whose support is smaller than a certain amount (10, 15, 30, and 50), which may indicate that the rules are not significant. 
As expected, we observe a trade-off between support and sparsity; when the constraint on MAX\_SPARSITY is relaxed, the cardinality of the rule increases and the rule becomes less interpretable, however, at the same time, support increases which improves the confidence in the resulting rule. 
Overall, the average cardinality is quite low, and the support is quite high. 


\begin{table}[]
\begin{tabular}{l|rrrrrr}
Formulation    &Support    &Cardinality    &Support$\leq$10    &Support$\leq$15    &Support$\leq$30    &Support$\leq$50\\
\hline
Max Sparsity                    &239.61    &2.89    &961    &1273    &1984    &2692\\
Max Support + 0    &444.76    &2.89    &468    &629    &931    &1344\\
Max Support + 1 &804.93    &3.62    &121    &184    &307    &483\\
Max Support + 2 &1096.63    &4.39    &21    &37    &81    &126\\
\hline
\end{tabular}
\caption{Comparison of consistent rules generated using different formulations.} \label{tab:comparison_rules} 
\end{table}
\fi

\begin{figure}
\centering
\includegraphics[width=0.80\linewidth]{rule_example_font20.png}
\qquad
\includegraphics[width=\linewidth]{rule3d.png}
\caption{\textit{Top:} an explanation for Observation 6 that has support of 700 observations; \textit{Bottom:} an explanation for Observation 1005 that has support of 990 observations.}
\label{fig:rule2d}
\end{figure}

\begin{figure*}[h]
 \includegraphics[width=\linewidth]{CaseBased.png}
  \caption{Case-based explanations.}
  \label{fig:CaseBased}
\end{figure*}
\paragraph{Optimization procedure for the challenge.} In an actual deployed system, generating rules could be done offline for each user, since users' credit information infrequently changes over time. In contrast, in our code, we wanted to allow the user the ability to interact with the system to see how explanations are generated for any possible new observation. Therefore, we wanted to limit the running time for generating explanations to provide a reasonably short response. 

To this end, we first created a database of summary-explanations using the FICO dataset. We created summary-explanations for maximal sparsity, and maximal support subject to sparsity constraints of +0, +1, and +2 of optimal. We did the same for 10K additional random observations. When a user clicks to generate an explanation, the database is scanned, and the sparsest rule whose support is greater than ten is returned. Otherwise, if no rules were found, the maximal sparsity optimization problem is solved. If the support of the returned rule is greater than 10, that solution is returned. Otherwise, the maximal support optimization is solved, consecutively relaxing the constraint on the maximal sparsity. If rules with sufficiently large support were not found, the procedure is repeated with minimal support set to 5 (instead of 10). Beyond this, an error message is displayed if no summary-explanations were found because the observation is an outlier; there is no rule characterizing it.

\iffalse
We note that the above approach is quite general and other alternatives of these basic formulations can be used. For example, optimizing both sparsity and support in the same objective function provides an alternative way for controlling the support/sparsity tradeoff. 
\fi

Figure~\ref{fig:rule2d} illustrates the tradeoff between simplicity and coverage for two rules generated by \texttt{SetCoverExplanation}. The rule on the left is 2-dimensional, and the rule on the right involves three dimensions.



%\begin{figure}
%\centering
%\fbox{\includegraphics[width=0.55\linewidth]{rule3d.png}}
%\caption{It explains observation 28 and has support of 1074 observations.}
%\label{fig:rule3d}
%\end{figure}

\subsection{Case-based explanations}\label{sub:consistent-cases}
%\textcolor{red}{
%YARON: the interface we only use case-based explanations using consistent rules. Should we move it to section 3.3?
%\\
%This is Chaofan. I have moved this section to 3.3. It just doesn't make sense to have it in 2.2.
%}

%\textcolor{red}{Fix me}
%Here we present another popular form of explanation, case-based explanations. %\citep{schank2014inside}.
Given a previously unseen case, we can identify similar cases from the FICO dataset to assess the prediction made by our global model for the unseen case. To do this, we find all the cases in the dataset that satisfy the consistent rule-based explanation for the unseen case (obtained by \texttt{SetCoverExplanation}). We then rank these cases according to how many binary features (see Section~\ref{gen_inst} for how we obtain the binary features) they share with the unseen case and present the five highest-ranked similar cases to the user. Figure~\ref{fig:CaseBased} gives an example of a case-based explanation: our visualization contains a table showing the current case (top row) and previous cases that are most closely related to the current case (all other rows). 
%\textcolor{blue}{Highlighted are features whose binary values coincide with the explained case (for example, in the binary representation of the feature ExternalRiskEstimate, the values 56,59,61, and 63 coincide).}
%All of the presented cases satisfy the consistent rule-based explanation from \texttt{SetCoverExplanation}.

%Our visualization contains a table showing the current case (top row) and previous cases that are most closely related to the current case (all other rows). All of the presented cases satisfy the rule-based explanations from \texttt{SetCoverExplanation}. Cases are sorted according to a distance metric that counts the number of identical features in the binary representation. See Figure~\ref{fig:CaseBased} for example case-based explanations.



\section{Thoughts}
%\textbf{Related work:} Several other entrants for the same competition produced beautiful visualization tools, including \cite{Sanjeeb2018}, \cite{Rory2018}, and \cite{Steffen2018}. In particular, \cite{Sanjeeb2018} used column generation to efficiently search over an exponential number of candidate conjunctive or disjunctive clauses without the need for heuristic rule mining. \cite{Rory2018} proposed positive counterfactuals and introduced several weighting strategies to generate more understandable counterfactuals. \cite{Steffen2018} created a multifaceted black-box model explanation to enhance the explainability of machine learning models and demonstrated their results with a beautiful visualization tool. %\textcolor{red}{Add a couple of sentences about what they did.}

\textbf{Competition Judging and Lessons Learned:}
Since the judging procedure was not announced in advance, none of the entrants knew prior to submitting their entries what the judging criteria would be. There were two evaluations: one created by the competition organizers, and an evaluation by FICO itself. 

As it turned out, in the first evaluation by the competition organizers, the competition's judging procedure for the challenge focused essentially on the \textit{ease of calculating} the explanation; judges were provided with partial explanations for only four observations, and asked to predict the black box model's predictions for these four observations, for both global and local predictions. Judges were not permitted to use any of the visualization tools submitted by any of the entrants. 

Generally, visualization tools are particularly useful for \textit{counterfactual reasoning}: users of the visualization tools can determine in real time what happens to the predictions when a feature changes by adjusting it directly. Since the judges were not able to use any of the visualization tools, they were not able to reason this way.

More importantly, the judges were not able to evaluate the \textit{fidelity} of any of the local models in representing their global model, for any of the competition entries. This means that local models that were poorly fitted to the global models may have received high scores. (Also, it is not clear how our entry was provided to the judges since all predictions -- from both our globally interpretable model and the summary-explanations -- are both local and global predictions for every observation. If our rule-based explanations were provided as both local and global predictions, then they may have been easier to calculate than the global model.)

Unfortunately, this meant that the judging team was not able to judge the major criteria for explainability: fidelity of the explanation, or counterfactual reasoning. 

As far as we know, none of the other competition entrants aimed to produce a globally interpretable model. Other entrants followed the competition instructions, which were to create a black box model and explain it. This is unfortunate, due to serious risks for using explainable black boxes rather than globally interpretable models \citep{Rudin18}.

The second evaluation of the competition was performed by FICO itself, and not by the competition organizers. We do not have details on how the entries were judged. Our entry was ranked first by FICO's criteria, earning the \textit{FICO recognition prize} for the competition. This allowed us to understand that FICO actually did value the globally interpretable model above the black box when given a choice between them.

There are some clear lessons learned from this competition. First, \textit{it is too often assumed that black boxes are necessary when they are not}. In many cases, black boxes are the mechanism by which a company profits -- this fuels what has been called ``the colossal asymmetry between societal cost and private gain in the rollout of automated systems" \citep{Powles2018}. The case of credit scoring is a key example -- if the dataset from FICO is at all representative, our work demonstrates that \textit{perhaps we do not need black box models for credit scoring}.

A second lesson learned is that explainability should not always be judged according to ease of computation. Additive models are known to be interpretable/explainable but are not easy to compute by hand. It is well-known that sparsity, while useful for some applications, is not the only measure of interpretability \citep{Freitas:2014ic}. Further, aspects such as fidelity of explanation, counterfactual reasoning, and more generally, the ability of the user to understand how variables are combined \textit{jointly} to form predictions are often more important than only ease of calculation.

\textbf{Discussion and Future Work:} There are several possible direct extensions to our work. Methods like RiskSLIM \citep{UstunRu2017KDD} could make the subscale scores more interpretable by restricting to integer coefficients. Our visualization interface could be extended to be much fancier, like \cite{Ming2018} for rule-list exploration. 

An essential topic important to lending decisions but not handled by this work is averting bias towards protected groups. 
Fairness is a major concern in credit ratings, and even lately people have found that lending decisions are horribly biased.\footnote{https://www.bloomberg.com/markets/fixed-income} 
However, for other protected classes beyond age, credit rating agencies do not have reliable or accurate demographic data for consumers or borrowers on most credit products. 
%For mortgages, some demographic information is collected. However, none of that data is available for use in credit scoring systems because for every other financial product, this data is not collected. 
The Consumer Financial Protections Bureau (CFPB) has developed a proxy for ethnicity based off of last name and geographical location, but that kind of data is not easy to simulate. If these data were able to be obtained or estimated, we could add constraints to the model so that it obeys a desired definition of fairness, though there is not a single definition of algorithmic fairness that is yet widely accepted, and multiple definitions of fairness conflict with each other, making them impossible to satisfy simultaneously.
%It is an open question as to whether or not this proxy is statistically valid. A lending institution may apply this proxy to ensure their lending practices aren't creating disparate impact because it is accepted by the CFPB. In summary, since they don't have reliable demographics data or proxies, they say it is hard explicitly to test for disparate impact or other bias in the model.  

Missing data is another important topic that we did not discuss in depth. Missing data is commonly imputed, but imputation of missing data can be problematic, because decisions are then made on data that can be incorrect. Another way to handle missing data is to create many models, each of which relies on a separate subset of variables. Then, if a variable is missing, we can use a model that does not rely on that variable. The approach presented in this work could be used for any of those models; once the user reports which variables are missing, we envision that the appropriate model would be automatically selected by a visualization interface. In this paper, we do not impute missing data, and individuals do not accrue points on any subscale for the \textit{values of} missing variables,  but since we have an indicator for whether certain variables are missing, our model sometimes leverages \textit{the fact that} the variable was missing to help make better predictions. Missingness is not at random, and thus whether a variable is missing can reasonably contribute to accuracy in prediction. 

Since the FICO dataset does not seem to require a black box for good performance, perhaps many other applications in finance also do not require a black box \citep[see, e.g.][]{RudinRa2019}. The answer to this hypothesis remains unclear. However, challenges like the one initiated by FICO can help us to determine the answer to this important question.

\textbf{Link:}
Our interface can be found here:\\ \href{http://dukedatasciencefico.cs.duke.edu}{http://dukedatasciencefico.cs.duke.edu}


%\section*{Appendix: Login Information}
%The web interface for our system can be found at: \href{http://dukedatasciencefico.cs.duke.edu}{http://dukedatasciencefico.cs.duke.edu} \\
%with username dukedatascience and password OxNaUTsSjH0GQ

% \bibliographystyle{plainnat}
% \bibliography{reference}





%\end{document}

